Effective matrix model for deconfinement in pure gauge theories

We construct matrix models for the deconfining phase transition in SU(N) gauge theories, without dynamical quarks, at a nonzero temperature T. We generalize models with zero and one free parameter to study a model with two free parameters: besides perturbative terms ~T^4, we introduce terms ~T^2 and ~T^0. The two N-dependent parameters are determined by fitting to data from numerical simulations on the lattice for the pressure, including the latent heat. Good agreement is found for the pressure in the semi-quark gluon plasma (QGP), which is the region from Tc, the critical temperature, to about ~4 Tc. Above ~1.2 Tc, the pressure is a sum of a perturbative term, ~ +T^4, and a simple non-perturbative term, essentially just a constant times ~ -Tc^2 T^2. For the pressure, the details of the matrix model only enter within a very narrow window, from Tc to ~1.2 Tc, whose width does not change significantly with N. Without further adjustment, the model also agrees well with lattice data for the 't Hooft loop. This is notable, because in contrast to the pressure, the 't Hooft loop is sensitive to the details of the matrix model over the entire semi-QGP. For the (renormalized) Polyakov loop, though, our results disagree sharply with those from the lattice. Matrix models provide a natural and generic explanation for why the deconfining phase transition in SU(N) gauge theories is of first order not just for three, but also for four or more colors. Lastly, we consider gauge theories where there is no strict order parameter for deconfinement, such as for a G(2) gauge group. To agree with lattice measurements, in the G(2) matrix model it is essential to add terms which generate complete eigenvalue repulsion in the confining phase.

==> G2plots.tex <==
%cpkaApril07
%rdp, Feb29
\section{\Gtwo ~results}\label{sec:g2plots}

In this section, we show numerical results for the pressure and 
eigenvalues for a G(2) gauge group. We assume that the
thermodynamic potential is of the form
%
\bea
{\cal V}_{tot}^{\Gtwo}(q_1,q_2) &=& T^4 \left(
\Vpt^{\Gtwo}(q_1,q_2) \; + \; \Vnpt(q_1,q_2,t) \right) \\
 \Vpt^{\Gtwo}(q_1,q_2) &=& \pi^2\left[\; - \; \frac{14}{45} \; + \;
     \frac{4}{3} \; V_2^{\Gtwo}(q_1,q_2) \right] 
        \label{eq:Vpt_G2}
\eea
%
Here, $V_2^{\Gtwo}(q_1,q_2)$ is a function found by computing to one loop
order in $G(2)$ in a background $A_0$ field,
%
\bea
V_{n}^{\Gtwo}(q_1,q_2) &=& B_{2 n}(q_1) + B_{2 n}(q_2) \nonumber \\
&+& B_{2 n}(q_1+q_2)
    + B_{2 n}(q_1-q_2) + B_{2 n}(2q_1+q_2) + B_{2 n}(q_1+2q_2)\; .
 \label{eq:V2G2}
\eea
%
As before, the $B_{2 n}(q)$'s are, up to an overall constant,
given by Bernoulli polynomials,
%
\beq
B_{2 n}(q) = |q|_1^n \, (1-|q|_1)^n~~~~,~~~
|q|_1 \equiv |q|~\mathrm{mod}~1~ \; .
\eeq
%

As shown in the previous section, we have a large degree of freedom
in choosing the non-perturbative potential. To illustrate the possible
behavior, we consider two cases.

The first we term a ``pure $\Gtwo$'' model,
%
\bea
\Vnpt^{\Gtwo}(q_1,q_2,t) &=& - \frac{4}{3} \frac{\pi^2}{t^2} \left[ \;
			   c_1^{\Gtwo}  \; V_1^{\Gtwo}(q_1,q_2) \; + \;
			   c_2^{\Gtwo} \; V_2^{\Gtwo}(q_1,q_2) \; + \;
			   c_3 \; \right]  \label{eq:Vnpt_G2} \; ,
\eea
%
where $t = T/T_c$.
This is the exact analogue of what we did for $SU(N)$: we introduce
terms $\sim B_2$ to ensure that the theory is always in a Higgs phase.
Terms $\sim B_4$ appear in the
perturbative potential, so we also introduce them in the
non-perturbative potential.   The point is that the $q$'s always enter
as expected from the perturbative computation in $\Gtwo$.
To simplify the discussion, we term the ``minimal'' $\Gtwo$ model
that where $c_2^{\Gtwo} = 0$.

The problem is that as we shall show, this natural extension of $SU(N)$
to $G(2)$ gives a result in manifest contradiction to lattice results.
There is a first order transition, but the low temperature phase is
deconfined, with a nonzero expectation value for the Polyakov loop.

To avoid this, we enforce eigenvalue repulsion in the low
temperature phase, {\it by hand}, by
introducing additional terms to the non-perturbative potential.
These are characteristic not of $G(2)$,
but of $SU(7)$. Another way trying to avoid the deconfining low $T$ phase is to add the fundamental representation  as argued in the  previous section. For example, consider the following potential,
which involves five parameters,
%
\bea
\Vnpt^{\SUseven}(q_1,q_2,t) = - \frac{4}{3} \frac{\pi^2}{t^2} \left[ \right.
\; &c_1^{\SUseven}&  \; V_1^{\SUseven}(q_1,q_2)  
\; + \; c_1^{\Gtwo}  \; V_1^{\Gtwo}(q_1,q_2)  \nonumber \\
\; + \; &c_2^{\Gtwo}& \left.
\; V_2^{\Gtwo}(q_1,q_2)  \; +  \; c_2^{\SUseven} \; V_2^{\SUseven}(q_1,q_2) 
\; + \; c_3 \; \right]~.  \label{eq:Vnpt_SU7}
\eea
%
The $SU(7)$ potentials are given by
%
\bea
V^{SU(7)}_{n}(q_1,q_2) &=&
B_{2n}(2 q_1) + B_{2n}(2 q_2) + B_{2 n}(2 q_1 + 2 q_2) \nonumber\\
&+& 2 \, B_{2 n}(q_1 - q_2) + 2 \, B_{2 n}(2 q_1 + q_2) 
+ 2 \, B_{2 n}(q_1 + 2 q_2) \nonumber\\
&+& 4 \, B_{2 n}(q_1) + 4\, B_{2 n}(q_2) + 4 \, B_{2 n}(q_1 + q_2) \; .
\label{SU7nonpert_2}
\eea
%

As before, we have two conditions amongst the coefficients.  One is
that the transition occurs at $T_c$ (i.e.,at $t=1$).  The other is
that the pressure vanishes at $T_c$.  Thus Eq.\ (\ref{eq:Vnpt_SU7}) has
not five, but three free parameters.  In this three dimensional space,
there are many types of transitions possible.  Typically, there is at
least one first order transition to a low temperature phase which is
deconfined, with nonzero expectation values for the fundamental and
adjoint Polyakov loops.  We also found cases with two separate first
order transitions, where all phases are deconfined.

Instead of mapping out the full three dimensional space, we limit
ourselves to the simplest model which appears to give a result which
is consistent with the lattice results.  The obvious choice is
%
\beq
c_1^{\Gtwo} \; = \; 0 \;\;\; ; \;\;\;
c_2^{\Gtwo} \; = \; 1 \; .
\eeq
%
We term the resulting potential a ``$\SUseven$'' model.  Basically,
it is contrived to suppress all $G(2)$ terms at $T_c$.  Since
$V_2^{\Gtwo}$ enters perturbatively, we tune $c_2^{\Gtwo} = 1$
in the non-perturbative potential, so that they cancel identically
at $T_c$.  In contrast, as $V_1^{\Gtwo}$ only enters into the non-perturbative
potential, we set its coefficient to vanish.
Making these two choices, we are then led to a $SU(7)$ model with one
free parameter, which we choose as $c_2^{\SUseven}$.

In $G(2)$, the fundamental representation is related to the $SU(3)$
embedding as
${\bf 7} = {\bf 1} + {\bf 3} + \overline{{\bf 3}}$
\cite{Holland:2002vk}, so that
the fundamental loop is given by
\cite{Wellegehausen:2009rq, *Wellegehausen:2010ai, *Wellegehausen:2011sc}
%
\beq
{\ell}_{\bf{7}} = \frac{1}{7}
\left( 1 + 2 \, \cos(2 \pi q_1) + 2 \, \cos(2 \pi q_1) 
+ 2 \, \cos(2 \pi (q_1+q_2) ) \right) \; .
\eeq
%
The adjoint representation is related to the $SU(3)$ embedding as
${\bf 14} = {\bf 3} + \overline{{\bf 3}} + {\bf 8}$, so that 
\cite{Wellegehausen:2009rq, *Wellegehausen:2010ai, *Wellegehausen:2011sc}
%
\bea
{\ell}_{\bf{14}} = \frac{1}{7}
\left( 1 \right. &+& 
\cos(2 \pi q_1) + \cos(2 \pi q_1) + \cos(2 \pi (q_1+q_2) )\\
&+& \left.\cos(2 \pi (q_1 - q_2)) + \cos(2 \pi (2 q_1 +  q_2) ) 
+ \cos(2 \pi (q_1+ 2 q_2) \right) \; .
\eea
%

\begin{figure}
\includegraphics{weylchamberg2.eps}
\vspace*{-0.61cm}
\caption{ Blow up of right panel in fig.(\ref{fig:g2lattice}).%The semi-circle is the locus of vanishing Polyakov loop. Note on the curve  the fully repulsive $SU(7)$ vacuum $Y_c(7)=((1/7)(3,-2,-1)$ at $r=0$ and the line connecting it to the origin on which the degenerate vacuum $r_c(7)=9/19$ lies.
The magenta points are the location of the degenerate vacua of the $V_{tot}^{G(2)}$
adjoint potential or "pure $G(2)$ model", as shown in fig.(\ref{fig:G2q1q2}).   }
\label{fig:weylchamberg2} 
\end{figure}





\begin{figure}[htbp]
\includegraphics[width=0.45\textwidth]{ell1_G2npt.eps}
\includegraphics[width=0.45\textwidth]{ellAdj_G2npt.eps}
\caption{\label{fig:G2Loops}Expectation value of the Polyakov loop in
  the fundamental (left) and adjoint (right) representations of \Gtwo,
  respectively, for four cases: the minimal \Gtwo\ model (dotted line),
  a model with a term involving the fundamental loop, and for two
  models with confining \SUseven vacua, $\sim c_2^{SU(7)}$.  Note that
  for the minimal \Gtwo model, the fundamental loop is {\it non}zero
  below $T_c$.}
\end{figure}
In Fig.~\ref{fig:G2Loops}
we plot the expectation value of the Polyakov loop
in the fundamental ${\bf 7}$ and in the adjoint ${\bf 14}$
representation, respectively.
In both cases, the minimal $G(2)$ model gives nonzero expectation values
for the loops below $T_c$.  In contrast, and
really because we have forced the theory to behave so, the 
\SUseven\ models do not.

\begin{figure}[htbp]
\includegraphics{q1q2_G2npt.eps}
\vspace*{-1cm}
\caption{\label{fig:G2q1q2}Expectation values of the {\it eigenvalues}
  of the \Gtwo~Polyakov loop for the minimal \Gtwo~model (dotted and
  dashed-dotted lines) and for the \SUseven~model with $c_2^\SUseven=-2$.}
\end{figure}

It is interesting to note the evolution of the {\it eigenvalues} of
the \Gtwo~Polyakov loop with temperature. This is shown in
Fig.~(\ref{fig:G2q1q2}). We find that they remain close to although not
exactly on the \SUseven\ path $|q_1/q_2|=2$.

\begin{figure}[htbp]
\includegraphics{press_G2npt.eps}
\vspace*{-1cm}
\caption{\label{fig:G2pressure}Pressure as a function of temperature
  for the \Gtwo\ potentials.}
\end{figure}
Fig.~(\ref{fig:G2pressure}) shows the pressure obtained from the
\Gtwo\ model.


\begin{figure}[htbp]
\includegraphics[width=0.45\textwidth]{e-3p_T4_G2npt.eps}
\includegraphics[width=0.45\textwidth]{e-3p_T2_G2npt.eps}
\vspace*{-.5cm}
\caption{\label{fig:G2e-3p} Interaction measure $(e-3p)/T^4$  (left)
  and rescaled interaction measure $(e-3p)/T^2T_c^2$ (right)
for the \Gtwo~potentials.}
\end{figure}
In Fig.~(\ref{fig:G2e-3p}) we show the interaction measure $e-3p$
obtained from our \Gtwo\ potentials. In our model with \SUseven
non-perturbative potential $(e-3p)/T^4$ does not exhibit a peak and
drops rather slowly towards high temperature. On the other hand, the
``pure \Gtwo'' model as well as the model with the term involving the
loop in the fundamental representation do exhibit a peak in the
interaction measure; also, the rescaled interaction measure is
approximately flat at high $T$.



\subsection{Adding the fundamental ${\bf 7}$ to the pure $G(2)$ potential}
In this section we return to the pure \Gtwo model but add a term
involving the loop in the fundamental representation as given in
\eq (\ref{eq:addingvector}). That is, we take the
model~(\ref{eq:Vnpt_G2}) and add 
%
\beq \label{eq:G2FundPot}
-d_2V^{G(2){\bf 7}}_2({\bf q}_{G2}) = - d_2{4\pi^2\over {3
    t^2}}\bigg(B_4(q_1)+B_4(q_2)+B_4(q_3)\bigg).  
\eeq 
%
We find that
this term weakens the first-order transition and reduces the
expectation values of both the fundamental and the adjoint loop at
$T_c^+$ as seen in \figs
\ref{fig:G2LoopsA},\ref{fig:G2LoopsB}. Presumably the model is driven
towards an end point of a line of first-order transitions.  The
term~(\ref{eq:G2FundPot}) also leads to much smaller expectation
values of both loops below $T_c$. The interaction measure $\Delta$
away from $T_c$ behaves very similar to the pure \Gtwo model
without~(\ref{eq:G2FundPot}) considered previously.






==> su6su7.tex <==
%cpkaApril07
\section{Numerical solution of the model for six and seven colors}
\la{sec:su67}

For these two groups the space where the trace of the fundamental loop
is real is three dimensional.  For $SU(6)$ the results are interesting
because of the issue whether the transition has an intermediate $Z(2)$
invariant phase or whether it is absent like in $SU(4)$.

Furthermore the symplectic group $Sp(6)$ is the pseudo-real part of
$SU(6)$, and $Sp(6)$~\cite{Holland:2003kg} is the dual (by exchanging
short and long roots) of $SO(7)$. As already remarked in section
(\ref{sec:effectivepotential}) the one loop approximation to both
groups is therefore related by duality. As long as we take the same,
i.e. duality related, representations in the non-perturbative
potentials we have formally this duality. Formally because the the
coefficients $c_1, c_2,~\mbox{ etc.}$ should be the same, and this
must be determined by lattice measurements.


The results for $SU(7)$ are interesting because of their relevance for
the $G(2)$ (and $SO(7)$ ) confining state, discussed in section
({\ref{sec:weyl}})and (\ref{sec:g2plots}).


\begin{figure}
\includegraphics[width=15cm]{su67realtrace.eps}
\caption{\label{fig:su67realtrace} The three dimensional subsspaces
  $(q_1,q_2,q_3)$ where $\Tr{\bf L}=0$, in panel (a) for $SU(6)$ , in
  panel (b) for $SU(7)$. The planes where the various powers of ${\bf
    L}$ are given in panel (a). }
\end{figure}


==> weyl_notes <==
The problem is that as we shall show, this natural extension of $SU(N)$
to $G(2)$ gives a result in manifest contradiction to lattice results.
There is a first order transition, but the low temperature phase is
deconfined, with a nonzero expectation value for the Polyakov loop.


To avoid this, we enforce eigenvalue repulsion in the low
temperature phase, {\it by hand}, by
introducing additional terms to the non-perturbative potential.
These are characteristic not of $G(2)$,
but of $SU(7)$. Another way trying to avoid the deconfining low $T$ phase is to add the fundamental representation  as argued in the  previous section. For example, consider the following potential,
which involves five parameters,
%
\bea
\Vnpt^{\SUseven}(q_1,q_2,t) = - \frac{4}{3} \frac{\pi^2}{t^2} \left[ \right.
\; &c_1^{\SUseven}&  \; V_1^{\SUseven}(q_1,q_2)  
\; + \; c_1^{\Gtwo}  \; V_1^{\Gtwo}(q_1,q_2)  \nonumber \\
\; + \; &c_2^{\Gtwo}& \left.
\; V_2^{\Gtwo}(q_1,q_2)  \; +  \; c_2^{\SUseven} \; V_2^{\SUseven}(q_1,q_2) 
\; + \; c_3 \; \right]~.  \label{eq:Vnpt_SU7}
\eea
%
The $SU(7)$ potentials are given by


As before, we have two conditions amongst the coefficients.  One is
that the transition occurs at $T_c$ (i.e.,at $t=1$).  The other is
that the pressure vanishes at $T_c$.  Thus Eq.\ (\ref{eq:Vnpt_SU7}) has
not five, but three free parameters.  In this three dimensional space,
there are many types of transitions possible.  Typically, there is at
least one first order transition to a low temperature phase which is
deconfined, with nonzero expectation values for the fundamental and
adjoint Polyakov loops.  We also found cases with two separate first
order transitions, where all phases are deconfined.


